Bridging the Gap: Studio-like Avatar Creation from a Monocular Phone Capture

Creating photorealistic avatars for individuals traditionally involves extensive capture sessions with complex and expensive studio devices like the LightStage system. While recent strides in neural representations have enabled the generation of photorealistic and animatable 3D avatars from quick phone scans, they have the capture-time lighting baked-in, lack facial details and have missing regions in areas such as the back of the ears. Thus, they lag in quality compared to studio-captured avatars. In this paper, we propose a method that bridges this gap by generating studio-like illuminated texture maps from short, monocular phone captures. We do this by parameterizing the phone texture maps using the $W^+$ space of a StyleGAN2, enabling near-perfect reconstruction. Then, we finetune a StyleGAN2 by sampling in the $W^+$ parameterized space using a very small set of studio-captured textures as an adversarial training signal. To further enhance the realism and accuracy of facial details, we super-resolve the output of the StyleGAN2 using carefully designed diffusion model that is guided by image gradients of the phone-captured texture map. Once trained, our method excels at producing studio-like facial texture maps from casual monocular smartphone videos. Demonstrating its capabilities, we showcase the generation of photorealistic, uniformly lit, complete avatars from monocular phone captures. The project page can be found at http://shahrukhathar.github.io/2024/07/22/Bridging.html

==> _constants.tex <==
\def\paperID{1834}
\def\confName{ECCV}
\def\confYear{2024}

\def\paperTitle{Bridging the Gap: Studio-like Avatar Creation from a Monocular Phone Capture}

\def\authorBlock{
    ShahRukh Athar\thanks{Work done while interning at Meta} \qquad
    Author 2\footnotemark[1] \qquad
    Author 3 \\
    Institute \\
    {\tt\small \{email, addresses\}@inst.edu}
}

\newif\ifreview \newcommand{\review}{\reviewtrue}
\newif\ifarxiv \newcommand{\arxiv}{\arxivtrue}
\newif\ifcamera \newcommand{\cameraready}{\cameratrue}
\newif\ifrebuttal \newcommand{\rebuttal}{\rebuttaltrue}


==> cvpr_rebutt_header.tex <==
\ifreview \usepackage[review]{cvprrebutt} \fi
\ifarxiv \usepackage[pagenumbers]{cvprrebutt} \fi
\ifrebuttal \usepackage[rebuttal]{cvprrebutt} \fi
\ifcamera \usepackage{cvprrebutt} \fi

\input{macros}  %

\usepackage{xr-hyper}

\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}

\makeatother
\newcommand*{\myexternaldocument}[1]{
    \externaldocument{#1}
    \addFileDependency{#1.tex}
    \addFileDependency{#1.aux}
}

\definecolor{cvprblue}{rgb}{0.21,0.49,0.74}
\usepackage[pagebackref,breaklinks,colorlinks,citecolor=cvprblue]{hyperref}
\usepackage[capitalize]{cleveref}

\crefname{section}{Sec.}{Secs.}
\crefname{table}{Table}{Tables}
\crefname{figure}{Fig.}{Figs.}

\frenchspacing
\newcommand{\rone}{\textbf{\textcolor{orange}{R1}} }
\newcommand{\rtwo}{\textbf{\textcolor{violet}{R2}} }
\newcommand{\rthree}{\textbf{\textcolor{blue}{R3}} }


==> tables/OptAbaTex.tex <==
\begin{table}[h]
\begin{center}
\small
\scalebox{0.85}{
\begin{tabular}{lcccr}
\toprule
  \midrule
  Models  & Full Network opt & Opt8 (Ours)  & Opt16    \\
\midrule
 FaceID \(\downarrow\) & \(5.01e-4\) &  \(\mathcolorbox{yellow}{4.31e-4}\) & \(\mathcolorbox{pink}{4.30e-4}\) \\
 \midrule
 KID \(\downarrow\) &  \(\mathcolorbox{pink}{1.36e-3}\) &  \(\mathcolorbox{yellow}{1.42e-3}\) & \(1.63e-3\) \\
\bottomrule
\end{tabular}}
\caption{\small{Ablation of optimization resolution.  \mathcolorbox{pink}{\text{Best}} and \mathcolorbox{Yellow}{\text{Second Best}} scores are highlighted. } }

\label{tab:opt_aba}
\vspace{-0.5cm}
\end{center}
\end{table}


==> tables/faceIDLpipsAba.tex <==
\begin{table}[h]
\begin{center}
\small
\scalebox{0.85}{
\begin{tabular}{l{c}p{2cm}{c}p{2.5cm}{c}p{3.5cm}}
\toprule
  \midrule
  Models  & Full Loss & w/o \(\mathcal{L}_{FaceID}\)  & w/o \(\mathcal{L}_{FaceID}\) and  \(\mathcal{L}_{Percp}\)    \\
\midrule
 FaceID \(\downarrow\) & \(\mathcolorbox{pink}{5.36e-4}\) &  \(\mathcolorbox{yellow}{1.33e-3}\) & \(2.79e-3\) \\
\bottomrule
\end{tabular}}
\caption{\small{Ablation of Losses.  \mathcolorbox{pink}{\text{Best}} and \mathcolorbox{Yellow}{\text{Second Best}} scores are highlighted.  Note: These are the results of \(\GMug\) without the facial details added by our diffusion model } }


\label{tab:faceid_lpips_aba}
\vspace{-0.5cm}
\end{center}
\end{table}

